Extracting Novel Facts from Tables for Knowledge Graph Completion (Extended version)

We propose a new end-to-end method for extending a Knowledge Graph (KG) from tables. Existing techniques tend to interpret tables by focusing on information that is already in the KG, and therefore tend to extract many redundant facts. Our method aims to find more novel facts. We introduce a new technique for table interpretation based on a scalable graphical model using entity similarities. Our method further disambiguates cell values using KG embeddings as additional ranking method. Other distinctive features are the lack of assumptions about the underlying KG and the enabling of a fine-grained tuning of the precision/recall trade-off of extracted facts. Our experiments show that our approach has a higher recall during the interpretation process than the state-of-the-art, and is more resistant against the bias observed in extracting mostly redundant facts since it produces more novel extractions.

==> intuition.tex <==
%!TEX root = main.tex

\section{Intuition} % (fold)

% \begin{figure}[tb] \centering
% \includegraphics[width=0.8\linewidth]{img/overview} \caption{Approach overview
% with its main components.} \label{fig:overview} \end{figure}

Our approach applies three operations in a sequence, as shown in
Fig.~\ref{fig:overview}: The first operations pre-processes the input table to
determine whether it is suitable for extracting novel triples. The second one
interprets the table, i.e., maps the rows and columns to concepts in $\cK$.
Finally, the third operations extracts (novel) facts from the table so they can
be added to $\cK$.

\leanparagraph{Preprocessing} Not all tables are suitable to extract factual
information. We are interested in tables that describe entities; like the one
reported in Fig.~\ref{fig:method}. First, we identify the key-column (if any)
using the heuristics proposed by~\cite{Ritze2015MatchingHT} which consists of
selecting the column with most unique non-numeric values breaking ties by
choosing the leftmost one. This heuristics works well in practice so we apply it
without modifications. Only the tables with valid key columns are considered
since these are the only ones for which we can (potentially) extract factual
knowledge.

\leanparagraph{Table Interpretation} We apply a novel procedure to link the rows
and columns in the table to entities and relations in $\cK$ respectively. This is
the most important task in the pipeline because these links are crucial for
performing slot-filling.

Inline with other methods, we assume that the entities described in the rows are
similar to each other according to some unspecified criterion. It is important
that the similarity between entities is computed accurately because it is
precisely this value that later allows the system to select certain mappings
instead of others. Both \tkmatch and \tableminer consider two entities as
similar if they are instances of the same class. In principle this is an
effective choice, but it becomes suboptimal when the KG does not contain the
relevant class or when the similarity is defined over different attributes.

To overcome these limitations, we introduce a more general similarity function
which considers all shared attributes between two entities, and then employ a
statistical inference procedure to maximise the coherence between the
assignments. We use a PGM as statistical framework to infer likelihood scores
between rows and candidate mentions, and employ Loopy Belief Propagation
(LBP)~\cite{koller2009probabilistic} as inferencing method to change these
scores depending on how the various candidates are similar to each other. 
% For
% instance, suppose that there are two rows $\rho_1$ and $\rho_2$. Row $\rho_1$ can be
% mapped to entity $e_{11}$ with a likelihood score of $p_{11}$ and to entity
% $e_{12}$ with score $p_{12}$. Similarly, $\rho_2$ maps to entities $e_{21}$ and
% $e_{22}$ with scores $p_{21}$ and $p_{22}$ respectively. In this case, LBP will
% change the scores $p_{11},p_{12},p_{21},p_{22}$ s.t. $p_{1x}>p_{1y}$ and
% $p_{2z}>p_{2w}$ if the similarity $sim(e_{1x},e_{2z})$ is higher than
% $sim(e_{1y},e_{2w})$.

The scores returned by LBP indicate which are the assignments that maximise the
coherence between the entities. We combine these scores with other ones that
measure the syntactic overlap between the labels of the candidate entities (and
their attributes) and the content of the row. The score obtained by this
combination is used to rank the candidate entities and to select the one with
the highest score.

Since the scores for the entity candidates consider all shared neighbours and
not only class instantiation, our method can deal with a larger variety of
tables. This is beneficial because it leads to higher recall and thus can
improve the extraction of novel information.
%For instance,
%the two candidates in Fig.~\ref{fig:method}b do share the commonality that
%they are American satirical films, which is expressed by having the same
%attribute \emph{(subject, American\_satirical\_film)}. Since this attribute does
%not express class instantiation, it is not considered.

\leanparagraph{Slot filling} Finally, we proceed with the extraction of novel
triples from the content of attribute columns. Suppose that the previous operation
has mapped the content of row $i$ and non-key column $j$ to entity $e_i$ and
relation $\rel_j$ respectively. If we manage to associate the content of the cell
at coordinates $(i,j)$ to an entity $e_{i,j}$, then we can construct the triple
$\langle e_i, \rel_j, e_{i,j} \rangle$ and add it to $\cK$. To this end, we first
retrieve from $\cK$ all entities with a label that is similar to the content of
the cell. In case this operation returns multiple candidates, we make use of the
context that we have already acquired to rank them. Namely, we know already that
$e_{i,j}$ should be linked to $e_i$ through $\rel_j$. Therefore, we rank the
candidates depending on the likelihood that such link exists. To compute the
likelihood scores of potential links, we use the embeddings computed by
TransE~\cite{transe}. After the candidates are re-ranked, we select the one with
the highest likelihood score and return the extracted triple.

